Constraining the Infalling Envelope Models of Embedded Protostars: BHR 71 and its Hot Corino

The collapse of the protostellar envelope results in the growth of the protostar and the development of a protoplanetary disk, playing a critical role during the early stages of star formation. Characterizing the gas infall in the envelope constrains the dynamical models of star formation. We present unambiguous signatures of infall, probed by optically thick molecular lines, toward an isolated embedded protostar, BHR 71 IRS1. The three dimensional radiative transfer calculations indicate that a slowly rotating infalling envelope model following the "inside-out" collapse reproduces the observations of both HCO$^{+}$ $J=4\rightarrow3$ and CS $J=7\rightarrow6$ lines, and the low velocity emission of the HCN $J=4\rightarrow3$ line. The envelope has a model-derived age of 12000$\pm$3000 years after the initial collapse. The envelope model underestimates the high velocity emission at the HCN $J=4\rightarrow3$ and H$^{13}$CN $J=4\rightarrow3$ lines, where outflows or a Keplerian disk may contribute. The ALMA observations serendipitously discover the emission of complex organic molecules (COMs) concentrated within a radius of 100 au, indicating that BHR 71 IRS1 harbors a hot corino. Eight species of COMs are identified, including CH$_{3}$OH and CH$_{3}$OCHO, along with H$_{2}$CS, SO$_{2}$ and HCN $v_{2}=1$. The emission of methyl formate and $^{13}$C-methanol shows a clear velocity gradient within a radius of 50 au, hinting at an unresolved Keplerian rotating disk.

==> com_id.tex <==
\begin{deluxetable*}{r l l l l l l}
 \tabletypesize{\scriptsize}
 \tablecaption{Line Identification \label{tbl:line_id}}
 \tablewidth{\textwidth}
 \tablehead{\colhead{Line No.} & \colhead{Formula} & \colhead{Name} & \colhead{Frequency (MHz)} & \colhead{Transition$^{a}$} & \colhead{log(Einstein-A)} & \colhead{$E_{\rm u}$ (K)}}
 \startdata
 \multicolumn{7}{c}{HCN~\jj{4}{3}} \\
 \hline
 2  & \tmethanol                      & Methanol           &  354445.95(0.05)      & [4, 1, 3]$\rightarrow$[3, 0, 3]                                         &  1.274(-4) & 43.71   \\
 3  & \acetaldehyde$~{\rm v}_{t}=1$   & Acetaldehyde       &  354457.6646(0.0409)  & [18, 2, 16]$\rightarrow$[17, 2, 15]                                     &  1.585(-3) & 374.97  \\
 3  & HCN$~{\rm v}_{2}=1$             & Hydrogen cyanide   &  354460.4346(0.0007)  & \J=4$\rightarrow$3                                                      &  1.869(-3) & 1066.90 \\
 4  & \ethylcyanide                   & Ethyl cyanide      &  354476.6596(0.0015)  & [40, 3, 38]$\rightarrow$[39, 3, 37]                                     &  3.767(-3) & 361.47  \\
 5  & \acetaldehyde$~{\rm v}_{t}=1$   & Acetaldehyde       &  354522.7114(0.1995)  & [6, 6, 1]$\rightarrow$[7, 5, 3]                                         &  3.184(-6) & 304.34  \\
 5  & \methylamine                    & Methylamine        &  354528.4832(0.0057)  & [Sym, \J, \K]=[B$_2$, 8, 2]$\rightarrow$[B$_1$, 7, 2]                   &  2.156(-5) & 92.76   \\
 6  & \methylamine                    & Methylamine        &  354600.5152(29.979)  & [Sym, \J, \K]=[B$_2$, 8, 5]$\rightarrow$[B$_1$, 7, 5]                   &  1.399(-5) & 174.05  \\
 6  & \methylamine                    & Methylamine        &  354600.5152(29.979)  & [Sym, \J, \K]=[B$_1$, 8, 5]$\rightarrow$[B$_2$, 7, 5]                   &  1.399(-5) & 174.05  \\
 6  & \methylamine                    & Methylamine        &  354600.5152(29.979)  & [Sym, \J, \K]=[B$_1$, 8, 6]$\rightarrow$[B$_2$, 7, 6]                   &  1.016(-5) & 216.84  \\
 6  & \methylamine                    & Methylamine        &  354600.5152(29.979)  & [Sym, \J, \K]=[B$_2$, 8, 6]$\rightarrow$[B$_1$, 7, 6]                   &  1.016(-5) & 216.84  \\
 7  & \methylformate                  & Methyl formate     &  354608.0913(0.003)   & [33, 0, 33]$\rightarrow$[32, 1, 32]                                     &  1.097(-4) & 293.10  \\
 7  & \methylformate                  & Methyl formate     &  354608.0919(0.003)   & [33, 1, 33]$\rightarrow$[32, 1, 32]                                     &  6.792(-4) & 293.10  \\
 7  & \methylformate                  & Methyl formate     &  354608.0923(0.003)   & [33, 0, 33]$\rightarrow$[32, 0, 32]                                     &  6.792(-4) & 293.10  \\
 7  & \methylformate                  & Methyl formate     &  354608.0928(0.003)   & [33, 1, 33]$\rightarrow$[32, 0, 32]                                     &  1.097(-4) & 293.10  \\
 \hline
 \multicolumn{7}{c}{\hcop~\jj{4}{3}} \\
 \hline
 9  & \methanol                       & Methanol           &  356626.667(0.016)    & [\J, \K]= [23, 4]$\rightarrow$[22, 5]                                   &  8.041(-5) & 727.83  \\
 10 & \acetone                        & Acetone            &  356658.4123(0.0187)  & [27, 10, 17]$\rightarrow$[26, 11, 16], Sym=EA                           &  1.215(-3) & 274.98  \\
 10 & \acetone                        & Acetone            &  356658.4780(0.0187)  & [27, 11, 17]$\rightarrow$[26, 10, 16], Sym=EA                           &  1.215(-3) & 274.98  \\
 10 & \acetone                        & Acetone            &  356658.5351(0.0184)  & [27, 10, 17]$\rightarrow$[26, 11, 16], Sym=AE                           &  1.215(-3) & 274.98  \\
 10 & \acetone                        & Acetone            &  356658.6016(0.0184)  & [27, 11, 17]$\rightarrow$[26, 10, 16], Sym=AE                           &  1.215(-3) & 274.98  \\
 11 & \acetone                        & Acetone            &  356675.1969(0.0814)  & [19, 13, 6]$\rightarrow$[18, 12, 7]                                     &  6.123(-4) & 157.74  \\
 12 & \methylformatev                 & Methyl formate     &  356686.906(0.1)      & [29, 6, 24]$\rightarrow$[28, 6, 23]                                     &  6.584(-4) & 468.78  \\
 13 & \dmethanol                      & Methanol           &  356697.9372(0.0099)  & [9, 2, 8]$\rightarrow$[9, 0, 9]                                         &  3.536(-6) & 131.85  \\
 % 14 &   \dimethylether                    & Dimethyl ether     &  356705.1704(0.0214)     &   [\J, \Ka, \Kc, vibSym=EA]=[8, 4, 5]$\rightarrow$[7, 3, 5]              &  7.33(-5)    &   55.27   \\
 14 & \dimethylether                  & Dimethyl ether     &  356705.204(0.004)    & [8, 4, 4]$\rightarrow$[7, 3, 5], Sym=AE                                 &  9.249(-5) & 55.27   \\
 % 15 &   \dimethylether                    & Dimethyl ether     &    356712.9312(0.0128)        &     [\J, \Ka, \Kc, vibSym=EA]=[8, 4, 5]$\rightarrow$[7, 3, 5]                      &     6.255(-5)    &     55.266  \\
 15 & \dimethylether                  & Dimethyl ether     &  356712.951(0.002)    & [8, 4, 5]$\rightarrow$[7, 3, 5], Sym=EE                                 &  6.255(-5) & 55.27   \\
 15 & \methylformate                  & Methyl formate     &  356711.841(0.1)      & [29, 17, 12]$\rightarrow$[28, 17, 11]                                   &  4.561(-4) & 448.21  \\
 15 & \methylformate                  & Methyl formate     &  356711.841(0.1)      & [29, 17, 13]$\rightarrow$[28, 17, 11]                                   &  4.561(-4) & 448.21  \\
 16 & \dimethylether                  & Dimethyl ether     &  356724.457(0.003)    & [8, 4, 4]$\rightarrow$[7, 3, 5], Sym=AA                                 &  2.095(-4) & 55.27   \\
 16 & \dimethylether                  & Dimethyl ether     &  356724.864(0.003)    & [8, 4, 5]$\rightarrow$[7, 3, 5], Sym=AE                                 &  1.17(-4)  & 55.27   \\
 18 & \acetone                        & Acetone            &  356729.9828(0.0153)  & [27, 10, 17]$\rightarrow$[26, 11, 16], Sym=EE                           &  1.215(-3) & 275.00  \\
 19 & $\rm SO_{2}$                    & Sulfur dioxide     &  356755.1899(0.0014)  & [10, 4, 6]$\rightarrow$[10, 3, 7]                                       &  3.281(-4) & 89.83   \\
 20 & CH$_{3}$C$^{15}$N               & Methyl cyanide     &  356761.0470(0.002)   & [\J, \K]=[20, 1]$\rightarrow$[19, 1]                                    &  3.962(-3) & 186.97  \\
 22 & \dmethanol                      & Methanol           &  356796.1421(0.0034)  & [8, 6, 3]$\rightarrow$[7, 6, 2]                                         &  6.277(-5) & 234.12  \\
 22 & \dmethanol                      & Methanol           &  356796.1421(0.0034)  & [8, 6, 2]$\rightarrow$[7, 6, 1]                                         &  6.277(-5) & 234.12  \\
 \hline
 \multicolumn{7}{c}{CS~\jj{7}{6}} \\
 \hline
 25 & \acetone                        & Acetone            &  342780.0345(0.0357)  & [17, 17, 1]$\rightarrow$[16, 16, 0]                                     &  1.85(-3)  & 147.05  \\
 25 & \acetone                        & Acetone            &  342780.0361(0.0357)  & [17, 17, 0]$\rightarrow$[16, 16, 1]                                     &  1.85(-3)  & 47.05   \\
 26 & \dmethanol                      & Methanol           &  342935.6452(0.0118)  & [17, 2, 16]$\rightarrow$[17, 1, 17]                                     &  1.227(-4) & 342.83  \\
 27 & $\rm H_{2}CS$                   & Thioformaldehyde   &  342946.4239(0.0500)  & [10, 0, 10]$\rightarrow$[9, 0, 9]                                       &  6.08(-4)  & 90.59   \\
 \hline
 \multicolumn{7}{c}{\htcn~\jj{4}{3}} \\
 \hline
 29 & \tmethanol                      & Methanol           &  345132.599(0.05)     & [4, 0, 4]$\rightarrow$[3, 1, 3]                                         &  8.239(-5) & 35.76   \\
 31 & \methylformatev                 & Methyl formate     &  345148.04(0.1)       & [28, 6, 23]$\rightarrow$[27, 6, 22], Sym=A                              &  5.947(-4) & 451.66  \\
 32 & \methylformatev                 & Methyl formate     &  345162.544(0.1)      & [11, 8, 3]$\rightarrow$[10, 7, 3], Sym=E                                &  7.091(-5) & 269.30  \\
 33 & \ethanol                        & gauche-Ethanol     &  345173.9493(0.0112)  & [\J, \Ka, \Kc, $v_t$]=[7, 7, 1(0), 0]$\rightarrow$[6, 6, 1(0), 1]$^b$   &  2.515(-4) & 139.90  \\
 36 & \ethanol                        & gauche-Ethanol     &  345229.238(0.05)     & [\J, \Ka, \Kc, $v_t$]=[21, 1, 21, 0]$\rightarrow$[20, 1, 20, 0]         &  3.728(-4) & 241.55  \\
 39 & \methylformatev                 & Methyl formate     &  345248.21(0.1)       & [28, 10, 19]$\rightarrow$[27, 10, 18], Sym=E                            &  5.481(-4) & 492.90  \\
 40 & \acetone                        & Acetone            &  345256.0368(0.0368)  & [18, 15, 4]$\rightarrow$[17, 14, 3]                                     &  1.287(-3) & 150.83  \\
 43 & \ethanol                        & gauche-Ethanol     &  345295.3553(0.0022)  & [\J, \Ka, \Kc, $v_t$]=[21, 1, 21, 1]$\rightarrow$[20, 1, 20, 1]         &  3.731(-4) & 246.22  \\
 45 & \acetone                        & Acetone            &  345305.3651(0.0367)  & [18, 15, 3]$\rightarrow$[17, 14, 4]                                     &  1.288(-3) & 150.83  \\
 46 & \methanold$^{c}$                & Methanol           &  345319.587(0.359)    & [\J, \K, parity]=[8, 2, $-$]$\rightarrow$[8, 1, $+$]                    &  8.1 ($\mu^{2}\Sigma S$) & 100.14  \\
 48 & \dmethanol                      & Methanol           &  345398.9037(0.0112)  & [16, 2, 14]$\rightarrow$[15, 3, 13]                                     &  4.275(-5) & 310.21  \\
 49/50 & \ethanol                     & gauche-Ethanol     &  345408.1651(0.0022)  & [\J, \Ka, \Kc, $v_t$]=[21, 0, 21, 1]$\rightarrow$[20, 0, 20, 1]         &  3.743(-4) & 246.21  \\
 49/50 & CH$_{3}$Cl                   & Methyl chloride    &  345408.9874(0.0023)  & [\J, \K, $F$]=[13, 3, 12.5]$\rightarrow$[12, 3, 11.5]                   &  7.764(-4) & 183.47  \\
 53 & \methylformate                  & Methyl formate     &  345461.011(0.1)      & [28, 13, 15]$\rightarrow$[27, 13, 14], Sym=E                            &  4.94(-4)  & 351.85  \\
 54 & \methylformate                  & Methyl formate     &  345465.3445(0.0023)  & [16, 13, 4]$\rightarrow$[16, 12, 5], Sym=E                              &  2.513(-5) & 192.32  \\
 55 & \methylformatev                 & Methyl formate     &  345473.217(0.1)      & [28, 9, 19]$\rightarrow$[27, 9, 18], Sym=E                              &  5.626(-4) & 480.66  \\
 58 & \methylformate                  & Methyl formate     &  345486.602(0.1)      & [28, 13, 16]$\rightarrow$[27, 13, 15], Sym=E                            &  4.941(-4) & 351.85  \\
 60 & \methylformatev                 & Methyl formate     &  345510.004(0.1)      & [28, 9, 20]$\rightarrow$[27, 9, 19], Sym=A                              &  5.635(-4) & 480.51  \\
 61 & \methylformatev                 & Methyl formate     &  345571.314(0.1)      & [27, 5, 22]$\rightarrow$[26, 5, 21], Sym=E                              &  6.055(-4) & 480.80  \\
 \enddata
 \tablecomments{
  $^{a}$The typical quantum numbers are listed as [\J, \Ka, \Kc] unless specified. \\
  $^{b}$Two \textcolor{blue}{degenerated} transitions occur for \Kc=$1\rightarrow1$ and $0\rightarrow0$. \\
  $^{c}$\citet{1988ApJS...67..135A}.}
\end{deluxetable*}


==> coms_fitting.tex <==
\startlongtable
    \begin{deluxetable*}{r l l l l l l}
    \tabletypesize{\scriptsize}
    \tablecaption{Line Fitting \label{tbl:line_fitting}}
    \tablewidth{\textwidth}
    \tablehead{\colhead{Line No.} & \colhead{Frequency} & \colhead{Line Width} & \colhead{Integrated Flux} & \colhead{FWHM} & \colhead{PA} & \colhead{Method\tablenotemark{a}} \\
               \colhead{} & \colhead{[MHz]} & \colhead{[\kms]} & \colhead{[K~\kms]} & \colhead{[arcsec]} & \colhead{[deg.]} & \colhead{}}
    \startdata
    \multicolumn{5}{c}{\hcop~\jj{4}{3}} \\
    \hline
    1 & 354442.152 (0.068) & 3.5 (n/a) & 10.5 (0.3) & $0\farcs{61}\pm0\farcs{06}\times0\farcs{19}\pm0\farcs{04}$ & $160\fdg{76}\pm4\fdg{17}$ &  \\
    2 & 354445.941 (0.066) & 3.5 (n/a) & 11.3 (0.3) & $0\farcs{75}\pm0\farcs{06}\times0\farcs{17}\pm0\farcs{04}$ & $163\fdg{93}\pm2\fdg{37}$ &  \\
    3 & 354459.437 (0.060) & 6.6 (0.1) & 20.9 (0.3) & $0\farcs{48}\pm0\farcs{07}\times0\farcs{15}\pm0\farcs{09}$ & $163\fdg{4}\pm8\fdg{68}$ &  \\
    4 & 354476.565 (0.077) & 7.7 (0.2) & 16.3 (0.3) & $0\farcs{55}\pm0\farcs{11}\times0\farcs{18}\pm0\farcs{13}$ & $164\fdg{71}\pm10\fdg{74}$ &  \\
    5 & 354525.266 (0.133) & 9.1 (0.4) & 28.4 (0.9) & $0\farcs{67}\pm0\farcs{07}\times0\farcs{27}\pm0\farcs{07}$ & $16\fdg{21}\pm6\fdg{54}$ &  \\
    6 & 354600.954 (0.115) & 5.9 (0.2) & 15.1 (0.5) & $0\farcs{45}\pm0\farcs{11}\times0\farcs{22}\pm0\farcs{12}$ & $159\fdg{46}\pm23\fdg{35}$ &  \\
    7 & 354607.968 (0.020) & 3.8 (0.0) & 16.6 (0.2) & $0\farcs{53}\pm0\farcs{06}\times0\farcs{21}\pm0\farcs{06}$ & $166\fdg{72}\pm7\fdg{83}$ &  \\
    8 & 354622.820 (0.046) & 3.3 (0.1) & 8.0 (0.2) & $0\farcs{55}\pm0\farcs{14}\times0\farcs{23}\pm0\farcs{19}$ & $176\fdg{44}\pm19\fdg{62}$ &  \\
    \hline
    \multicolumn{5}{c}{HCN~\jj{4}{3}} \\
    \hline
    9 & 356626.832 (0.029) & 3.6 (0.1) & 10.1 (0.1) & $0\farcs{63}\pm0\farcs{1}\times0\farcs{25}\pm0\farcs{06}$ & $152\fdg{83}\pm8\fdg{26}$ &  \\
    10 & 356661.534 (0.120) & 7.5 (0.3) & 7.6 (0.2) & $0\farcs{62}\pm0\farcs{28}\times0\farcs{18}\pm0\farcs{14}$ & $161\fdg{76}\pm40\fdg{95}$ &  \\
    11 & 356675.940 (0.048) & 2.6 (0.1) & 2.1 (0.1) & $0\farcs{54}\pm0\farcs{27}\times0\farcs{17}\pm0\farcs{02}$\tablenotemark{a} & $132\fdg{84}\pm3\fdg{98}$\tablenotemark{a} &  \\
    12 & 356686.392 (0.077) & 3.0 (0.2) & 2.5 (0.1) & $0\farcs{45}\pm0\farcs{19}\times0\farcs{25}\pm0\farcs{06}$\tablenotemark{a} & $111\fdg{21}\pm14\fdg{71}$\tablenotemark{a} &  \\
    13 & 356697.008 (0.066) & 2.3 (0.1) & 3.2 (0.1) & $0\farcs{5}\pm0\farcs{26}\times0\farcs{26}\pm0\farcs{19}$ & $8\fdg{34}\pm37\fdg{52}$ &  \\
    14 & 356705.677 (0.052) & 2.4 (0.1) & 3.3 (0.1) & $0\farcs{34}\pm0\farcs{21}\times0\farcs{28}\pm0\farcs{19}$ & $175\fdg{46}\pm85\fdg{37}$ &  \\
    15 & 356712.809 (0.046) & 6.1 (0.1) & 14.2 (0.2) & $0\farcs{39}\pm0\farcs{13}\times0\farcs{29}\pm0\farcs{14}$ & $164\fdg{22}\pm58\fdg{56}$ &  \\
    16 & 356723.385 (0.122) & 2.9 (0.1) & 7.6 (0.1) & $0\farcs{58}\pm0\farcs{14}\times0\farcs{46}\pm0\farcs{14}$ & $23\fdg{16}\pm62\fdg{77}$ &  \\
    17 & 356726.062 (0.122) & 2.0 (0.1) & 4.4 (0.1) & $0\farcs{51}\pm0\farcs{11}\times0\farcs{22}\pm0\farcs{17}$ & $5\fdg{11}\pm17\fdg{43}$ &  \\
    18 & 356729.280 (0.122) & 1.9 (0.1) & 3.2 (0.1) & $0\farcs{46}\pm0\farcs{14}\times0\farcs{31}\pm0\farcs{19}$ & $42\fdg{73}\pm135\fdg{22}$ &  \\
    19 & 356755.672 (0.073) & 6.0 (0.2) & 15.7 (0.4) & $0\farcs{92}\pm0\farcs{11}\times0\farcs{27}\pm0\farcs{08}$ & $16\fdg{96}\pm4\fdg{35}$ &  \\
    20 & 356761.861 (0.143) & 3.1 (0.2) & 3.9 (0.4) & $0\farcs{47}\pm0\farcs{12}\times0\farcs{34}\pm0\farcs{15}$ & $30\fdg{08}\pm84\fdg{25}$ &  \\
    21 & 356767.248 (0.127) & 3.5 (0.3) & 4.4 (0.3) & $0\farcs{68}\pm0\farcs{25}\times0\farcs{28}\pm0\farcs{13}$ & $171\fdg{58}\pm30\fdg{66}$ &  \\
    22 & 356796.284 (0.080) & 4.9 (0.2) & 17.5 (0.6) & $0\farcs{66}\pm0\farcs{08}\times0\farcs{21}\pm0\farcs{07}$ & $175\fdg{06}\pm5\fdg{86}$ &  \\
    23 & 356831.654 (0.036) & 1.6 (0.1) & 1.5 (0.1) & $0\farcs{37}\pm0\farcs{24}\times0\farcs{21}\pm0\farcs{07}$\tablenotemark{a} & $53\fdg{03}\pm22\fdg{59}$\tablenotemark{a} &  \\
    24 & 356834.872 (0.047) & 3.2 (0.1) & 3.9 (0.1) & $0\farcs{43}\pm0\farcs{34}\times0\farcs{06}\pm0\farcs{26}$ & $170\fdg{54}\pm31\fdg{33}$ &  \\
    \hline
    \multicolumn{5}{c}{CS~\jj{7}{6}} \\
    \hline
    25 & 342782.231 (0.120) & 9.4 (0.3) & 13.3 (0.3) & $0\farcs{39}\pm0\farcs{17}\times0\farcs{06}\pm0\farcs{09}$ & $135\fdg{37}\pm25\fdg{55}$ &  \\
    26 & 342935.064 (0.123) & 3.7 (0.4) & 10.7 (0.7) & $0\farcs{54}\pm0\farcs{11}\times0\farcs{2}\pm0\farcs{14}$ & $167\fdg{08}\pm13\fdg{99}$ &  \\
    27 & 342946.841 (0.083) & 4.5 (0.2) & 11.8 (0.4) & $0\farcs{79}\pm0\farcs{14}\times0\farcs{4}\pm0\farcs{1}$ & $173\fdg{42}\pm12\fdg{93}$ &  \\
    28 & 342997.608 (0.072) & 6.8 (0.2) & 11.3 (0.3) & $0\farcs{28}\pm0\farcs{18}\times0\farcs{12}\pm0\farcs{09}$ & $142\fdg{82}\pm24\fdg{05}$ &  \\
    \hline
    \multicolumn{5}{c}{\htcn~\jj{4}{3}} \\
    \hline
    29 & 345132.485 (0.067) & 3.5 (0.1) & 11.2 (0.4) & $0\farcs{52}\pm0\farcs{06}\times0\farcs{26}\pm0\farcs{05}$ & $164\fdg{94}\pm10\fdg{2}$ &  \\
    30 & 345143.859 (0.108) & 3.5 (n/a) & 3.5 (0.1) & $0\farcs{47}\pm0\farcs{23}\times0\farcs{08}\pm0\farcs{11}$ & $145\fdg{08}\pm30\fdg{91}$ &  \\
    31 & 345149.137 (0.086) & 3.5 (n/a) & 4.0 (0.1) & $0\farcs{65}\pm0\farcs{19}\times0\farcs{03}\pm0\farcs{13}$ & $154\fdg{56}\pm9\fdg{46}$ &  \\
    32 & 345162.016 (0.164) & 8.7 (0.4) & 7.7 (0.3) & $0\farcs{31}\pm0\farcs{17}\times0\farcs{07}\pm0\farcs{27}$ & $16\fdg{09}\pm62\fdg{29}$ &  \\
    33 & 345179.918 (0.313) & 12.1 (0.6) & 9.8 (0.4) & $0\farcs{38}\pm0\farcs{08}\times0\farcs{26}\pm0\farcs{03}$\tablenotemark{a} & $160\fdg{0}\pm12\fdg{82}$\tablenotemark{a} &  \\
    34 & 345209.918 (0.244) & 5.4 (0.2) & 7.5 (0.2) & $0\farcs{46}\pm0\farcs{12}\times0\farcs{14}\pm0\farcs{09}$ & $166\fdg{95}\pm17\fdg{18}$ &  \\
    35 & 345219.314 (0.244) & 4.7 (0.2) & 3.7 (0.2) & $0\farcs{56}\pm0\farcs{12}\times0\farcs{3}\pm0\farcs{04}$\tablenotemark{a} & $10\fdg{47}\pm7\fdg{2}$\tablenotemark{a} &  \\
    36 & 345227.487 (0.244) & 5.1 (0.2) & 5.8 (0.2) & $0\farcs{51}\pm0\farcs{14}\times0\farcs{24}\pm0\farcs{1}$ & $142\fdg{58}\pm22\fdg{79}$ &  \\
    37 & 345235.814 (0.244) & 1.8 (0.2) & 1.9 (0.2) & $0\farcs{36}\pm0\farcs{22}\times0\farcs{27}\pm0\farcs{18}$ & $89\fdg{92}\pm86\fdg{65}$ &  \\
    38 & 345238.350 (0.244) & 1.6 (0.2) & 1.6 (0.2) & $0\farcs{55}\pm0\farcs{24}\times0\farcs{25}\pm0\farcs{18}$ & $125\fdg{19}\pm79\fdg{34}$ &  \\
    39 & 345246.534 (0.227) & 10.8 (0.7) & 9.6 (0.5) & $0\farcs{45}\pm0\farcs{19}\times0\farcs{37}\pm0\farcs{31}$ & $80\fdg{18}\pm84\fdg{75}$ &  \\
    40 & 345257.273 (0.169) & 5.5 (0.5) & 5.4 (0.3) & $0\farcs{78}\pm0\farcs{15}\times0\farcs{32}\pm0\farcs{03}$\tablenotemark{a} & $164\fdg{72}\pm4\fdg{37}$\tablenotemark{a} &  \\
    41 & 345283.154 (0.081) & 4.6 (0.2) & 9.2 (0.3) & $0\farcs{45}\pm0\farcs{09}\times0\farcs{24}\pm0\farcs{08}$ & $159\fdg{98}\pm20\fdg{63}$ &  \\
    42 & 345286.337 (0.051) & 1.1 (0.1) & 1.2 (0.2) & $0\farcs{58}\pm0\farcs{09}\times0\farcs{33}\pm0\farcs{03}$\tablenotemark{a} & $164\fdg{57}\pm6\fdg{85}$\tablenotemark{a} &  \\
    43 & 345295.184 (0.032) & 3.6 (0.1) & 6.7 (0.1) & $0\farcs{56}\pm0\farcs{11}\times0\farcs{14}\pm0\farcs{06}$ & $157\fdg{86}\pm8\fdg{35}$ &  \\
    44 & 345300.725 (0.052) & 2.9 (0.1) & 3.2 (0.1) & $0\farcs{54}\pm0\farcs{1}\times0\farcs{29}\pm0\farcs{03}$\tablenotemark{a} & $157\fdg{73}\pm6\fdg{49}$\tablenotemark{a} &  \\
    45 & 345306.003 (0.325) & 3.5 (n/a) & 3.7 (0.4) & $0\farcs{57}\pm0\farcs{21}\times0\farcs{24}\pm0\farcs{16}$ & $143\fdg{29}\pm33\fdg{65}$ &  \\
    46 & 345319.304 (0.113) & 3.5 (n/a) & 12.8 (0.5) & $0\farcs{52}\pm0\farcs{05}\times0\farcs{18}\pm0\farcs{06}$ & $168\fdg{3}\pm6\fdg{29}$ &  \\
    47 & 345324.737 (0.337) & 3.5 (n/a) & 4.8 (0.5) & $0\farcs{44}\pm0\farcs{06}\times0\farcs{3}\pm0\farcs{03}$\tablenotemark{a} & $147\fdg{78}\pm9\fdg{86}$\tablenotemark{a} &  \\
    48 & 345398.605 (0.056) & 3.6 (0.1) & 8.0 (0.2) & $0\farcs{48}\pm0\farcs{09}\times0\farcs{18}\pm0\farcs{08}$ & $156\fdg{98}\pm11\fdg{65}$ &  \\
    49 & 345406.474 (0.000) & 3.5 (n/a) & 4.2 (0.2) & $0\farcs{48}\pm0\farcs{07}\times0\farcs{34}\pm0\farcs{03}$\tablenotemark{a} & $158\fdg{65}\pm11\fdg{42}$\tablenotemark{a} &  \\
    50 & 345410.505 (0.062) & 3.5 (n/a) & 6.1 (0.2) & $0\farcs{39}\pm0\farcs{11}\times0\farcs{21}\pm0\farcs{14}$ & $165\fdg{46}\pm28\fdg{93}$ &  \\
    51 & 345444.943 (0.065) & 2.1 (0.2) & 4.2 (0.5) & $0\farcs{51}\pm0\farcs{09}\times0\farcs{21}\pm0\farcs{1}$ & $172\fdg{77}\pm13\fdg{21}$ &  \\
    52 & 345448.786 (0.405) & 6.9 (0.6) & 7.3 (0.8) & $0\farcs{44}\pm0\farcs{17}\times0\farcs{27}\pm0\farcs{19}$ & $108\fdg{81}\pm67\fdg{36}$ &  \\
    53 & 345459.960 (0.127) & 5.1 (0.3) & 6.8 (0.3) & $0\farcs{43}\pm0\farcs{05}\times0\farcs{39}\pm0\farcs{05}$\tablenotemark{a} & $53\fdg{47}\pm54\fdg{24}$\tablenotemark{a} &  \\
    54 & 345466.713 (0.147) & 3.5 (n/a) & 6.9 (0.3) & $0\farcs{42}\pm0\farcs{1}\times0\farcs{25}\pm0\farcs{16}$ & $7\fdg{53}\pm29\fdg{13}$ &  \\
    55 & 345473.520 (0.085) & 3.5 (n/a) & 4.0 (0.1) & $0\farcs{3}\pm0\farcs{13}\times0\farcs{22}\pm0\farcs{11}$ & $18\fdg{0}\pm85\fdg{98}$ &  \\
    56 & 345477.958 (0.131) & 3.5 (n/a) & 2.6 (0.1) & $0\farcs{5}\pm0\farcs{11}\times0\farcs{24}\pm0\farcs{02}$\tablenotemark{a} & $115\fdg{56}\pm4\fdg{91}$\tablenotemark{a} &  \\
    57 & 345485.493 (0.422) & 2.7 (0.7) & 4.0 (1.2) & $0\farcs{33}\pm0\farcs{1}\times0\farcs{11}\pm0\farcs{17}$ & $16\fdg{0}\pm35\fdg{58}$ &  \\
    58 & 345488.343 (0.375) & 2.2 (0.8) & 2.6 (1.4) & $0\farcs{43}\pm0\farcs{15}\times0\farcs{21}\pm0\farcs{16}$ & $17\fdg{49}\pm33\fdg{47}$ &  \\
    59 & 345492.056 (0.344) & 3.0 (0.6) & 2.9 (0.6) & $0\farcs{51}\pm0\farcs{1}\times0\farcs{41}\pm0\farcs{07}$\tablenotemark{a} & $52\fdg{49}\pm30\fdg{88}$\tablenotemark{a} &  \\
    60 & 345509.462 (0.067) & 4.9 (0.1) & 10.0 (0.2) & $0\farcs{29}\pm0\farcs{09}\times0\farcs{15}\pm0\farcs{09}$ & $1\fdg{13}\pm33\fdg{02}$ &  \\
    61 & 345546.657 (0.062) & 3.9 (0.1) & 3.8 (0.1) & $0\farcs{47}\pm0\farcs{21}\times0\farcs{05}\pm0\farcs{16}$ & $159\fdg{85}\pm33\fdg{31}$ &  \\
    62 & 345570.537 (0.100) & 3.3 (0.2) & 3.9 (0.2) & $0\farcs{48}\pm0\farcs{09}\times0\farcs{31}\pm0\farcs{04}$\tablenotemark{a} & $150\fdg{65}\pm11\fdg{41}$\tablenotemark{a} &  \\
    \enddata
    \tablenotetext{a}{One (or both) of the fitted FWHM is smaller than the beam size.
                      The fitted convolved sizes are shown instead.  Such situation is typical for weak lines close to 3$\sigma$}
    \tablecomments{
                   The uncertainty of line width are shown inside the prentice when the line width remains flexible for the fitting.
                   The FWHM lists the semi-major and semi-minor FWHM of the fitted 2D Gaussian profile,
                   while Figure~\ref{fig:com_morphology} shows the fitted shape.}
\end{deluxetable*}
